DETECT: Deep Trajectory Clustering for Mobility-Behavior Analysis

Identifying mobility behaviors in rich trajectory data is of great economic and social interest to various applications including urban planning, marketing and intelligence. Existing work on trajectory clustering often relies on similarity measurements that utilize raw spatial and/or temporal information of trajectories. These measures are incapable of identifying similar moving behaviors that exhibit varying spatio-temporal scales of movement. In addition, the expense of labeling massive trajectory data is a barrier to supervised learning models. To address these challenges, we propose an unsupervised neural approach for mobility behavior clustering, called the Deep Embedded TrajEctory ClusTering network (DETECT). DETECT operates in three parts: first it transforms the trajectories by summarizing their critical parts and augmenting them with context derived from their geographical locality (e.g., using POIs from gazetteers). In the second part, it learns a powerful representation of trajectories in the latent space of behaviors, thus enabling a clustering function (such as $k$-means) to be applied. Finally, a clustering oriented loss is directly built on the embedded features to jointly perform feature refinement and cluster assignment, thus improving separability between mobility behaviors. Exhaustive quantitative and qualitative experiments on two real-world datasets demonstrate the effectiveness of our approach for mobility behavior analyses.

==> background.tex <==
\section{Baseline Approaches} \label{sec:back}
\todo{Change sequence to trajectory here.}
In this section, we introduce the state-of-the-art trajectory clustering approaches which we will compare with DETECT in our experiments.
Traditional trajectory clustering approaches mostly adopt clustering methods used in sequence clustering, especially time series clustering~\cite{yuan2017review}. These approaches mainly utilize a clustering technique with a distance measurement designed for sequential data. These clustering approaches include centroid-based approaches (e.g., kMeans, kMedoids), density-based approaches (e.g., DBSCAN), hierarchical approaches (e.g., Agglomerative Clustering), and spectral clustering approach.
The distance measurements, however, are designed and adapted to different problems because the traditional pairwise distances such as Euclidean distance and Cosine distance are not applicable to variant-length sequences. Thus, researchers adopted measurements that could calculate distances between sequences with different lengths, e.g., Dynamic Time Warping (DTW) distance, Hausdorff distance, Longest Common SubSequence (LCSS) distance. In this section, we will briefly introduce some clustering approaches and distance measurements for sequences.

KMeans and DBSCAN are two popular clustering approaches. KMeans is a centroid-based clustering approach. The basic idea of kMeans is to find each instance the right cluster by assigning it to its nearest centroid and update these centroids. The algorithm assumes the number of clusters $k$ is provided and initializes k random centroids. Then the algorithm employs an iterative clustering process, each iteration includes two steps: a) every instance is assigned to the closest centroid, b) all centroids are updated by averaging the instances in the same cluster. Such iterations continue until a criterion is reached, e.g., the assignment of clusters does not change. Unlike kMeans, DBSCAN is a density-based clustering approach which does not require the knowledge of the number of clusters. It relies on the user's preference on the size and tightness of clusters. The algorithm defines reachability to determine if the instances are close enough to each other. In detail, $p$ is reachable to $q$ if $dist(p,q)<\epsilon$. Such reachability is transitive, i.e., $r$ is reachable to $q$ if $r$ is reachable to $p$ and $p$ is reachable to $q$. Thus the instances connected by the reachability form a cluster. Also, those instances not connected to any cluster will be marked as outliers. In this way, dense regions automatically generate clusters, and therefore the boundaries of clusters can be any shapes. This property makes DBSCAN sometimes preferable to kMeans since the boundaries of kMeans have to be convex shapes.

\todo{change "trajectory" to "sequence", or use a new notation other than x.}
In distance measurements for sequences, DTW is one designed to capture the shape of a sequence, by allowing warping among different timestamps. The algorithm is based on dynamic programming, which finds the best alignment between two trajectories and minimizes their distance. Different from the Euclidean distance, which computes the distance between two points at the same slice, DTW allows one point in sequence $s_1$ to find the matching point in sequence $s_2$ at a different slice, while keeping the order of the mapping. Figure \ref{fig:dtw} shows the difference between the DTW and Euclidean distances, as well as the DTW alignment between two sequences. Under the hood, the DTW distance between $s_1$ and $s_2$ is calculated by the recursive equation as shown in Equation~\eqref{eq:dtw}. An adaptive window (the blue area in Figure~\ref{fig:dtw2}) is often utilized to avoid over-distortion. We can observe in Figure~\ref{fig:dtw1} that the DTW distance is more capable than the Euclidean distance in capturing the shape and invariant to sequential shifts. 
\begin{equation}
\label{eq:dtw}
    DTW(i,j) = dist(s_1^{(i)}, s_2^{(j)}) + min\left\{\begin{matrix}
DTW(i-1, j)\\ 
DTW(i,j-1)\\ 
DTW(i-1, j-1)
\end{matrix}\right.
\end{equation}
LCSS is a distance measurement originally used for natural language sequences, where the task is finding the maximum length of common substrings between two sentences. To extend LCSS to numeric sequential data, a threshold $\epsilon$ has to be determined to measure the similarity between points from each sequence. Specifically, given two sequences $s_1, s_2$, we seek for the longest sub-sequences $s'_1 \subset s_1$, $s'_2 \subset s_2$, such that $|s'_1| = |s'_2|$, and all corresponding pair-wise distances between $s'_1$ and $s'_2$ are less or equal to $\epsilon$. The length of such subsequences is usually computed recursively as shown in Equation~\eqref{eq:lcss}. The length is usually normalized to $\frac{LCSS(s_1, s_2)}{min(|s_1|,|s_2|)}$, so variant lengths can be mapped to $[0,1]$. In addition, the calculated result describes the similarity between two trajectories. Thus to define a distance measurement, people usually define the LCSS distance as 
$1 - \frac{LCSS(s_1, s_2)}{min(|s_1|,|s_2|)}$. 
% Need better alignment of the equation
\begin{equation}
\label{eq:lcss}
\resizebox{0.43\textwidth}{!}{
    $LCSS(s_{1}^{(i)}, s_{2}^{(j)}) = \left \{ \begin{matrix}
0 & i=0\;  or \; j=0\\ 
1 + LCSS(s_{1}^{(i-1)}, s_{2}^{(j-1)}) & dist(s_{1}^{(i)}, s_{2}^{(j)}) \leq \epsilon\\ 
max(LCSS(s_{1}^{(i-1)}, s_{2}^{(j)}), LCSS(s_{1}^{(i)}, s_{2}^{(j-1)})) & otherwise
\end{matrix}\right.$

}
\end{equation}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.45\columnwidth}
        \centering
        \includegraphics[width = \columnwidth]{dtw1}
        \caption{}
        \label{fig:dtw1}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\columnwidth}
    \centering
        \includegraphics[width = \columnwidth]{dtw2}
        \caption{}
        \label{fig:dtw2}
    \end{subfigure}
    \caption{Alignment between two sequences: (a) difference between Euclidean and DTW (b) DTW alignment path~\cite{paparrizos2015k}}
    \label{fig:dtw}
\end{figure}

